Resistance boundaries of infinite networks

A resistance network is a connected graph $(G,c)$. The conductance function $c_{xy}$ weights the edges, which are then interpreted as conductors of possibly varying strengths. The Dirichlet energy form $\mathcal E$ produces a Hilbert space structure ${\mathcal H}_{\mathcal E}$ on the space of functions of finite energy. The relationship between the natural Dirichlet form $\mathcal E$ and the discrete Laplace operator $\Delta$ on a finite network is given by $\mathcal E(u,v) = \la u, \Lap v\ra_2$, where the latter is the usual $\ell^2$ inner product. We describe a reproducing kernel $\{v_x\}$ for $\mathcal E$ and used it to extends the discrete Gauss-Green identity to infinite networks: \[{\mathcal E}(u,v) = \sum_{G} u \Delta v + \sum_{\operatorname{bd}G} u \tfrac{\partial}{\partial \mathbf{n}} v,\] where the latter sum is understood in a limiting sense, analogous to a Riemann sum. This formula immediately yields a boundary sum representation for the harmonic functions of finite energy. Techniques from stochastic integration allow one to make the boundary $\operatorname{bd}G$ precise as a measure space, and give a boundary integral representation (in a sense analogous to that of Poisson or Martin boundary theory). This is done in terms of a Gel'fand triple $S \ci {\mathcal H}_{\mathcal E} \ci S'$ and gives a probability measure $\mathbb{P}$ and an isometric embedding of ${\mathcal H}_{\mathcal E}$ into $L^2(S',\mathbb{P})$, and yields a concrete representation of the boundary as a set of linear functionals on $S$.

==> energy-hilbert-space.tex <==
%%!TEX root = DGG.tex

\section{The energy Hilbert space}
\label{sec:energy-Hilbert-space}

In this section, we study the Hilbert space \HE of (finite-energy) voltage functions, that is, equivalence classes of functions $u:\verts \to \bC$ where $u \simeq v$ iff $u-v$ is constant. On this space, the energy form is an inner product, and there is a natural reproducing kernel $\{v_x\}_{x \in \verts}$ indexed by the vertices; see Corollary~\ref{thm:vx-is-a-reproducing-kernel}. Since we work with respect to the equivalence relation defined just above, most formulas are given with respect to differences of function values; in particular, the reproducing kernel is given in terms of differences with respect to some chosen ``origin''. Therefore, for any given \ERN, we fix a reference vertex $o \in \verts$ to act as an origin. It will readily be seen that all results are independent of this choice. When working with representatives, we typically abuse notation and use $u$ to denote the equivalence class of $u$. One natural choice is to take $u$ so that $u(o)=0$; a different but no less useful choice is to pick $k$ so that $v=0$ outside a finite set as discussed further in Definition~\ref{def:Fin}.

%Additionally, we show how the dipoles $\{v_x\}$ are related to the boundary structure of an \ERN in Theorem~\ref{thm:boundary-repn-for-harmonic}, and use them to construct and understand the boundaries of networks in \S\ref{sec:boundary-of-an-infinite-ERN}.

%The energy Hilbert space \HE will facilitate our study of the resistance metric $R$ in \S\ref{sec:effective-resistance-metric}. In particular, it provides an explanation for an issue stemming from the ``nonuniqueness of currents'' in certain infinite networks; see \cite{Lyons:ProbOnTrees, Thomassen90}. This disparity leads to differences between two apparently natural extensions of the effective resistance to infinite networks, which are greatly clarified by the geometry of Hilbert space. Also, \HE presents an analytic formulation of the type problem for random walks on an \ERN: transience of the random walk is equivalent to the existence of monopoles, that is, finite-energy solutions to a certain Dirichlet problem. In fact, this approach will readily allow us to obtain explicit formulas for effective resistance on integer lattice networks in \S\ref{sec:lattice-networks}, with applications to a physics problem of \cite{Pow76b} in \S\ref{sec:Magnetism-and-long-range-order}. 

%Henceforth, we will discuss \bC-valued functions on the vertices \verts, in contrast to the \bR-valued functions of the previous sections. However, $\cond=\ohm^{-1}$ will still be an \bR-valued (in fact, positive) function.

Let \one denote the constant function with value 1 and recall that $\ker \energy = \bC \one$. 

\begin{defn}\label{def:H_energy}\label{def:The-energy-Hilbert-space}
  The energy form \energy is symmetric and positive definite on $\dom \energy$. Then $\dom \energy / \bC \one$ is a vector space with inner product and corresponding norm given by
  \linenopax
  \begin{equation}\label{eqn:energy-inner-product}
    \la u, v \ra_\energy := \energy(u,v)
    \q\text{and}\q
    \|u\|_\energy := \energy(u,u)^{1/2}.
  \end{equation}
  The \emph{energy Hilbert space} \HE is the completion of $\dom \energy / \bC \one$ with respect to \eqref{eqn:energy-inner-product}.
\end{defn}

It can be checked directly that the above completion consists of (equivalence classes of) functions on \verts via an isometric embedding into a larger Hilbert space as in \cite{Lyons:ProbOnTrees,MuYaYo} or by a standard Fatou's lemma argument as in \cite{Soardi94}.

\begin{remark}[Three warnings about \HE] \hfill 
  \label{rem:elements-of-HE-are-technically-equivalence-classes}
  \begin{enumerate}
    \item \HE has no canonical o.n.b.; the usual candidates $\{\gd_x\}$ are not orthogonal by \eqref{eqn:energy-of-Diracs}, and typically their span is not even dense; cf. Corollary~\ref{thm:Diracs-not-dense}.
    \item Pointwise identities should not be confused with Hilbert space identities; see Remark~\ref{rem:Lap-defined-via-energy} and Lemma~\ref{thm:pointwise-identity-implies-adjoint-identity}.
    \item Multiplication operators are not generally Hermitian, as we show in the next lemma contrasts sharply with more familiar Hilbert spaces.
    \item There is no natural interpretation of \HE as an $\ell^2$-space of functions on the vertices \verts or edges \edges of $(\Graph,\cond)$.
  \end{enumerate}
  With regard to (4), it should be noted that \HE does contain the embedded image of $\ell^2(\verts,\gm)$ for a certain measure \gm, but this space is not typically dense, and almost never equal to \HE. Also, \HE embeds isometrically into a subspace of $\ell^2(\edges,\cond)$, but it generally nontrivial to determine whether a given element of $\ell^2(\edges,\cond)$ lies in this subspace. \HE may also be understood as a $\ell^2$ space of random variables \cite[\S15.1]{OTERN} or realized as a subspace of $L^2(S',\prob)$, where $S'$ is a certain space of distributions \cite{bdG}, but both of these constructions are beyond the scope of the present paper.
\end{remark}

\begin{lemma}\label{thm:multiplication-not-hermitian}
  If $\gf:\verts \to \bR$ and $M_\gf$ denotes the multiplication operator defined by $(M_\gf u)(x) = \gf(x) u(x)$, then $M_\gf$ is Hermitian if and only if $M_\gf = k\id$, for some $k \in \bR$. 
  \begin{proof}
    Choose any representatives for $u, v \in \HE$. From the formula \eqref{eqn:def:energy-form},
    \linenopax
    \begin{align*}%\label{eqn:}
      \la M_\gf u, v\ra_\energy
      &= \frac12 \sum_{x,y \in \verts} \cond_{xy} (\gf(x)u(x)v(x) - \gf(x)u(x)v(y) - \gf(y)u(y)v(x) + \gf(y)u(y)v(y)).
    \end{align*}
    By comparison with the corresponding expression, this is equal to $\la u, M_\gf v\ra_\energy$ iff $(\gf(y) - \gf(x))u(y)v(x) = (\gf(y) - \gf(x))u(x)v(y)$. However, since we are free to vary $u$ and $v$, it must be the case that \gf is constant and hence $\gf = 0$ in \HE. The converse is trivial.
  \end{proof}
\end{lemma}


\subsection{The evaluation operators $L_x$ and the reproducing kernel $\{v_x\}$}
\label{sec:L_x-and-v_x}

\begin{defn}\label{def:L_x}
  For any vertex $x \in \verts$, define the linear evaluation operator $L_x$ on \HE by
  \linenopax
  \begin{equation}\label{eqn:def:L_x}
    L_x u := u(x) - u(o).
  \end{equation}
  \glossary{name={$L_x$},description={evaluation functional; see $v_x$},sort=L,format=textbf}
\end{defn}

\begin{lemma}\label{thm:L_x-is-bounded}
  For any $x \in \verts$, one has $|L_x u | \leq k \energy(u)^{1/2}$, where $k$ depends only on $x$.
  \begin{proof}
    Since \Graph is connected, choose a path $\{x_i\}_{i=0}^n$ with $x_0=o$, $x_n=x$ and $\cond_{x_i,x_{i-1}}>0$ for $i=1,\dots,n$. For $k = \left(\sum_{i=1}^n \cond_{x_i,x_{i-1}}^{-1} \right)^{1/2}$, the Schwarz inequality yields
    \linenopax
    \begin{align*}
      |L_x u |^2
      = |u(x)-u(o)|^2
      &= \left|\sum_{i=1}^n \sqrt{\frac{\cond_{x_i,x_{i-1}}}{\cond_{x_i,x_{i-1}}}} (u(x_i)-u(x_{i-1}))\right|^2 
      %&\leq \left(\sum_{i=1}^n \frac1{\cond_{x_i,x_{i-1}}}\right) \left(\sum_{i=1}^n \cond_{x_i,x_{i-1}} (u(x_i)-u(x_{i-1}))^2\right) \\
      \leq k^2 \energy(u).
      \qedhere
    \end{align*}
  \end{proof}
\end{lemma}

\begin{defn}\label{def:vx}\label{def:energy-kernel}
  Let $v_x$ be defined to be the unique element of \HE for which
  \linenopax
  \begin{equation}\label{eqn:def:vx}
    \la v_x, u\ra_\energy = u(x)-u(o),
    \qq \text{for every } u \in \HE.
  \end{equation}
  This is justified by Lemma~\ref{thm:L_x-is-bounded} and Riesz's lemma.
  The family of functions $\{v_x\}_{x \in \verts}$ is called the \emph{energy kernel} because of Corollary~\ref{thm:vx-is-a-reproducing-kernel}.
  Note that $v_o$ corresponds to a constant function, since $\la v_o, u\ra_\energy = 0$ for every $u \in \HE$. Therefore, this term may be ignored or omitted.
\end{defn}

\begin{cor}\label{thm:vx-is-a-reproducing-kernel} \label{thm:vx-dense-in-HE}
  $\{v_x\}_{x \in \verts}$ is a reproducing kernel for \HE. Thus, $\spn\{v_x\}$ is dense in \HE.
  \begin{proof}
    Choosing representatives with $v_x(o)=0$, it is trivial to check that $\la v_x, v_y\ra_\energy = v_x(y) = \cj{v_y(x)}$ and then apply Aronszajn's Theorem \cite{Aronszajn50}. The energy kernel is clearly total, so density is immediate.
  \end{proof}
\end{cor}

There is a rich modern literature dealing with reproducing kernels and their manifold application to both continuous analysis problems (see e.g., \cite{AD06, AL08, AAL08, BV03, Zh09}), and infinite discrete stochastic models. One novel aspect of the present work is the use of ``relative'' (to the reference vertex $o$) reproducing kernels.

%\begin{defn}\label{def:reproducing-kernel}
%  Let $\sH$ be a Hilbert space of functions on $X$. An operator $S$ on \sH is said to have a \emph{reproducing kernel} $\{k_x\}_{x \in X} \ci \sH$ iff
%  \linenopax
%  \begin{equation}\label{eqn:def:reproducing-kernel}
%    (S v)(x) = \la k_x, v\ra_\sH,
%    \qq \forall x \in X, \forall v \in \sH.
%  \end{equation}
%  If $S$ is projection to a subspace $L \ci \sH$, then one says $\{k_x\}$ is a \emph{reproducing kernel for $L$}.
%  If $S=\id$, then \sH is a \emph{reproducing kernel Hilbert space} with kernel $k$.
%\end{defn}

%\begin{theorem}[Aronszajn's Theorem {\cite{Aronszajn50}}]
%  \label{thm:Aronszajn's-thm}
%  Let $\{f_x\}$ be a reproducing kernel for \sH. Define a sesquilinear form on the set of all finite linear combinations of these elements by
%  \linenopax
%  \begin{equation}\label{eqn:Aronszajn's-form}
%    \left\la \sum_x \gx_x f_x, \sum_y \gh_y f_y \right\ra
%    := \sum_x \cj{\gx_x} \gh_x f_x(y).
%  \end{equation}
%  Then the completion of this set under the form \eqref{eqn:Aronszajn's-form} is again \sH.
%\end{theorem}


\begin{comment}
  \label{rem:reproducing-kernel}
  Definition~\ref{def:energy-kernel} is justified by Corollary~\ref{thm:vx-is-a-reproducing-kernel}. In this paper, the functions $v_x$ will play a role analogous to fundamental solutions in PDE theory; see \S\ref{sec:analogy-with-complex-functions}. %In particular, they have a very close relation to the Green kernel, as described in \S\ref{sec:Green-function-and-operator}. 

  The functions $v_x$ are \bR-valued. This can be seen by first constructing the energy kernel for the Hilbert space of \bR-valued functions on \Graph, and then using the decomposition of a \bC-valued function $u = u_1 + \ii u_2$ into its real and imaginary parts. Alternatively, see Lemma~\ref{thm:vx-is-R-valued}.
  
  Reproducing kernels will help with many calculations and explain several of the relationships that appear in the study of \ERNs. They also extend the analogy with complex function theory discussed in \S\ref{sec:analogy-with-complex-functions}. The reader may find the references \cite{Aronszajn50,Yoo05,Jor83} to provide helpful background on reproducing kernels.
\end{comment}

\begin{remark}[Comparison to Kuramochi kernel]
  \label{rem:Kuramochi-kernel}
  After a first version of this paper was completed, the authors were referred to \cite{MuYaYo} in which the authors construct a reproducing kernel very similar to ours, which they call the Kuramochi kernel. Indeed, the Kuramochi kernel element $k_x$ corresponds to the representative of $v_x$ which takes the value 0 at $o$. This makes the Kuramochi kernel a reproducing kernel for the space of functions
  \linenopax
  \begin{align*}%\label{eqn:}
    \sD(\Graph;o) := \{u \in \dom \energy \suth u(o)=0\}.
  \end{align*} 
  As advantages of the present approach, we note that our formulation puts the Green kernel in the same space as the reproducing kernel. This will be helpful below; for example, the kernel elements $v_x$ and $f_x = \Phar v_x$ can be decomposed in terms of the Green kernel. See Definition~\ref{def:monopole} and Remark~\ref{rem:ranLap-vs-Fin}. The reader will find that we put the energy kernel to very different uses the Kuramochi kernel.
\end{remark}

\begin{remark}\label{rem:alternative-construction-of-HE}
  There is an alternative construction of \HE via techniques of von Neumann and Schoenberg \cite{vN32a,Schoe38a,Schoe38b}. The natural notion of distance on \Graph is the \emph{effective resistance metric} $R$, which is defined in terms of \energy. Because this metric is negative semidefinite, von Neumann's method gives an embedding $\gF: \Graph \to \sH$ of the metric space $(\Graph,R)$ into a Hilbert space \sH in such a way that $R(x,y) = \|\gF(x)-\gF(y)\|_\sH^2$. In \cite[\S6]{OTERN}, it is shown that $\gF(x) \mapsto v_x$ is a unitary isomorphism of \sH onto \HE.
\end{remark}

\begin{remark}[Probabilistic interpretation of $v_x$]
  \label{rem:interpretation-of-v_x}
  The energy kernel $\{v_x\}$ is intimately related to effective resistance distance $R(x,y)$. In fact, $R(x,o) = v_x(x) - v_x(o) = \energy(v_x)$ and similarly, $R(x,y) = \energy(v_x-v_y)$. This is discussed in detail in \cite{ERM}, but we give a brief summary here, to help the reader get a feeling for $v_x$. For a random walk (R.W.) started at the vertex $y$, let $\gt_x$ be the hitting time of $x$ (i.e., the time at which the random walk first reaches $x$) and define the function
  \linenopax
  \begin{align*}%\label{eqn:}
    u_x(y) = \prob[\gt_x < \gt_o | \text{ R.W. starts at $y$}].
  \end{align*}
  Here, the R.W. is governed by transition probabilities  $p(x,y) = \cond_{xy}/\cond(x)$; cf.~Remark~\ref{rem:transient-iff-monopoles}. One can show that $v_x = R(x,o) u_x$ is the representative of $v_x$ with $v_x(o)=0$. Since the range of $u_x$ is $[0,1]$, one has $0 \leq v_x(y) - v_x(o) \leq v_x(x) - v_x(o) = R(x,o)$. Many other properties of $v_x$ are similarly clear from this interpretation. For example, it is easy to compute $v_x$ completely on any tree.
\end{remark}


\subsection{The finitely supported functions and the harmonic functions}
\label{sec:The-role-of-Fin-in-HE}

\begin{defn}\label{def:Fin}
  For $v \in \HE$, one says that $v$ has \emph{finite support} iff there is a finite set $F \ci \verts$ for which $v(x) = k \in \bC$ for all $x \notin F$. Equivalently, the set of functions of finite support in \HE is 
  \linenopax
  \begin{equation}\label{eqn:span(dx)}
    \spn\{\gd_x\} = \{u \in \dom \energy \suth u(x)=k \text{ for some $k$, for all but finitely many } x \in \verts\},
  \end{equation}
  where $\gd_x$ is the Dirac mass at $x$, i.e., the element of \HE containing the characteristic function of the singleton $\{x\}$. It is immediate from \eqref{eqn:energy-of-Diracs} that $\gd_x \in \HE$.
  Define \Fin to be the closure of $\spn\{\gd_x\}$ with respect to \energy. 
\end{defn}

\begin{defn}\label{def:Harm}
  The set of harmonic functions of finite energy is denoted
  \linenopax
  \begin{equation}\label{eqn:Harm}
    \Harm := \{v \in \HE \suth \Lap v(x) = 0, \text{ for all } x \in \verts\}.
  \end{equation}
  Note that this is independent of choice of representative for $v$ in virtue of \eqref{eqn:def:laplacian}.
\end{defn}

\begin{lemma}\label{thm:<delta_x,v>=Lapv(x)}
  The Dirac masses $\{\gd_x\}_{x \in \verts}$ form a reproducing kernel for \Lap. That is, for any $x \in \verts$, one has $\la \gd_x, u \ra_\energy = \Lap u(x)$.
  \begin{proof}
    Compute $\la \gd_x, u \ra_\energy = \energy(\gd_x, u)$ directly from formula \eqref{eqn:def:energy-form}.
  \end{proof}
\end{lemma}

\begin{remark}\label{rem:Lap-defined-via-energy}
   Note that one can take the definition of the Laplacian to be the operator $A$ satisfying $\la \gd_x, u \ra_\energy = Au(x)$. This point of view is helpful, especially when distinguishing between identities in Hilbert space and pointwise equations. For example, if $h \in \Harm$, then $\Lap h$ and the constant function \one are identified in \HE because $\la u, \Lap h \ra_\energy = \la u, \one\ra_\energy = 0$, for any $u \in \HE$. However, one should not consider a (pointwise) solution of $\Lap u(x) = 1$ to be a harmonic function.
\end{remark}

\begin{lemma}\label{thm:vx-is-dipole}
  For any $x \in \verts$, $\Lap v_x = \gd_x - \gd_o$.
  \begin{proof}
    Using Lemma~\ref{thm:<delta_x,v>=Lapv(x)}, $\Lap v_x(y) = \la \gd_y, v_x\ra_\energy = \gd_y(x) - \gd_y(o) = (\gd_x-\gd_o)(y)$.
  \end{proof}
\end{lemma}

\begin{defn}\label{def:dipole}
  A \emph{dipole} is any $v \in \HE$ satisfying the pointwise identity $\Lap v = \gd_x - \gd_y$ for some vertices $x,y \in \verts$. It is clear from Lemma~\ref{thm:vx-is-dipole} that the energy kernel consists of dipoles, and that $v_x - v_y$ is always a finite-energy solution to $\Lap v = \gd_x - \gd_y$.
\end{defn}

Lemma~\ref{thm:<delta_x,v>=Lapv(x)} is extremely important. Since \Fin is the closure of $\spn\{\gd_x\}$, it implies that the finitely supported functions and the harmonic functions are orthogonal. This result is sometimes called the ``Royden Decomposition'' in honour of the analogous theory established by Royden for Riemann surfaces when it first appeared in \cite[Thm.~4.1]{Yamasaki79}. However, the result is incorrect as stated there and the following corrected form may also be found in \cite[\S{VI}]{Soardi94} or \cite[\S9.3]{Lyons:ProbOnTrees}.

\begin{theorem}\label{thm:HE=Fin+Harm}
  $\HE = \Fin \oplus \Harm$.
  \begin{proof}
    For all $v \in \HE$, Lemma~\ref{thm:<delta_x,v>=Lapv(x)} gives $\la \gd_x, v \ra_\energy = \Lap v(x)$. Since $\Fin = \spn\{\gd_x\}$, this equality shows $v \perp \Fin$ whenever $v$ is harmonic. Conversely, if $\la \gd_x, v \ra_\energy=0$ for every $x$, then $v$ must be harmonic. Recall that constants functions are 0 in \HE.
  \end{proof}
\end{theorem}

\begin{cor}\label{thm:Diracs-not-dense}
  $\spn\{\gd_x\}$ is dense in \HE iff $\Harm=0$.
\end{cor}

\begin{remark}\label{rem:Diracs-not-dense}
  Corollary~\ref{thm:Diracs-not-dense} is immediate from Theorem~\ref{thm:HE=Fin+Harm}, but we wish to emphasize the point, as it is not the usual case elsewhere in the literature and leads to unusual consequences, e.g., one may have
  \linenopax
  \begin{align*}%\label{eqn:}
    u \neq \sum_{x \in \verts} u(x) \gd_x, 
    \q \text{in \HE}.
  \end{align*}
  More precisely, $\|u - \sum_{x \in G_k} u(x) \gd_x\|_\energy$ may not tend to 0 as $k \to \iy$, for any exhaustion $\{G_k\}$. Part of the importance of the energy kernel $\{v_x\}$ arises from the fact that there is no other natural representing set for \HE. See also \cite[Lemma~3.1]{Yamasaki79} for a similar interesting implication. 
\end{remark}

\begin{defn}\label{def:ux}
  Let $f_x = \Pfin v_x$ denote the image of $v_x$ under the projection to \Fin. Similarly, let $h_x = \Phar v_x$ denote the image of $v_x$ under the projection to \Harm. 
\end{defn}

For future reference, we state the following immediate consequence of orthogonality.
\begin{lemma}\label{thm:repkernels-for-Fin-and-Harm}
  With $f_x = \Pfin v_x$, $\{f_x\}_{x \in \verts}$ is a reproducing kernel for \Fin, but $f_x \perp \Harm$. Similarly, with $h_x = \Phar v_x$, $\{h_x\}_{x \in \verts}$ is a reproducing kernel for \Harm, but $h_x \perp \Fin$.
\end{lemma}

While it may not be true that $v_y$ is in $\spn\{\gd_x\}$ (or even in its closure), 
the following result shows that $\gd_y$ is always in $\spn\{v_x\}$ when $\deg(y) < \iy$. 
    
\begin{lemma}\label{thm:dx-as-vx}
  For any $x \in \verts$, $\gd_x = \cond(x) v_x - \sum_{y \nbr x} \cond_{xy} v_y$.
  \begin{proof}
    Lemma~\ref{thm:<delta_x,v>=Lapv(x)} implies $\la \gd_x, u\ra_\energy = \la \cond(x) v_x - \sum_{y \nbr x} \cond_{xy} v_y, u\ra_\energy$ for every $u \in \HE$, so apply this to $u=v_z$, $z \in \verts$. Since $\gd_x, v_x \in \HE$, it must also be that $\sum_{y \nbr x} \cond_{xy} v_y \in \HE$.
  \end{proof}
\end{lemma}

\begin{remark}[Real and complex-valued functions on \verts]
  \label{rem:Real-and-complex-valued-functions-on-verts}
  While we will need complex-valued functions for some results obtained via spectral theory, it will usually suffice to consider \bR-valued functions because of the following lemma.
\end{remark}

\begin{lemma}\label{thm:vx-is-R-valued}
  The reproducing kernels $v_x, f_x, h_x$ are all \bR-valued functions.
  \begin{proof}
    Computing directly,
    \linenopax
    \begin{align*}
      \la \cj{v_z}, \cj{u}\ra_\energy
      &= \frac12\sum_{x,y \in \verts} (v_z(x)-v_z(y))(\cj{u}(x)-\cj{u}(y)) 
      %&= \cj{\frac12\sum_{x,y \in \verts} (\cj{v_z}(x)-\cj{v_z}(y))(u(x)-u(y))} \\
      = \cj{\la v_z, u\ra_\energy}.
    \end{align*}
    Then applying the reproducing kernel property,
    \linenopax
    \begin{align*}
      \cj{\la v_z, u \ra_\energy}
      = \cj{u(x)-u(o)} 
      = \cj{u}(x)-\cj{u}(o) 
      = \la v_z, \cj{u}\ra_\energy.
    \end{align*}
    Thus $\la \cj{v_z}, \cj{u}\ra_\energy = \la v_z, \cj{u}\ra_\energy$ for every $u \in \Harm$, and $v_z$ must be \bR-valued. The same computation applies to $f_z$ and $h_z$.
  \end{proof}
\end{lemma}

\begin{defn}\label{def:pointwise-convergence-in-HE}
  A sequence $\{u_n\} \ci \HE$ \emph{converges pointwise in \HE} iff $\exists k \in \bC$ such that $u_n(x)-u(x) \to k$, for all $x \in \verts$.
\end{defn}

\begin{lemma}\label{thm:E-convergence-implies-pointwise-convergence}
  If $\{u_n\}$ converges to $u$ in \energy, then $\{u_n\}$ converges to $u$ pointwise in \HE.
  \begin{proof}
    Define $w_n := u_n-u$ so that $\|w_n\|_\energy \to 0$. Then
    \linenopax
    \begin{align*}
      |w_n(x)-w_n(o)|
      = |\la v_x, w_n\ra_\energy|
      \leq \|v_x\|_\energy \cdot \|w_n\|_\energy
      \limas{n} 0,
    \end{align*}
    so that $\lim w_n$ exists pointwise and is a constant function.
  \end{proof}
\end{lemma}





==> paths.tex <==
%%!TEX root = RBIN.tex

\subsection{The boundary as equivalence classes of paths}
\label{sec:bdG-as-equivalence-classes-of-paths}

We are finally able to give a concrete representation of elements of the boundary. We continue to use the measure \quotprob from Theorem~\ref{thm:HE-isom-to-L2(S',P)}. %induced on the quotient $\Squoth $ as in Definition~\ref{def:quotprob}.  
Recall the Fock space representation of $L^2(\Schw',\prob)$ discussed in Remark~\ref{rem:Wiener-improves-Minlos}:
% if one were to reprove Theorem~\ref{thm:HE-isom-to-L2(S',P)} for $\sW$ defined only on \Harm, then \eqref{eqn:Minlos-expectation-integral} implies that we have a corresponding Fock space representation for the quotient:    
  \linenopax
  \begin{align}\label{eqn:Fock-repn-of-L2(S',P)-as-HE}
    L^2\left(\Squot,\quotprob\right) \cong \bigoplus_{n=0}^\iy \HE^{\otimes n}.
  \end{align}
  where $\HE^{\otimes 0} := \bC \one$ for a unit ``vacuum'' vector \one corresponding to the constant function, and $\HE^{\otimes n}$ denotes the $n$-fold \emph{symmetric} tensor product of \HE with itself. Observe that \one is orthogonal to \Fin and \Harm, but is not the zero element of $L^2(\Squoth,\quotprob)$.
  
\begin{lemma}\label{thm:int(u)=0-over-bdG}
  For all $v \in \Harm$, $\int_{\Squoth} v \, d\quotprob = 0$.
  \begin{proof}
     The integral $\int_{\Squoth} v \, d\quotprob = \int_{\Squoth} \one v \, d\quotprob$ is the inner product of two elements in $L^2(\Squoth,\quotprob)$ which lie in different (orthogonal) subspaces; see \eqref{eqn:Fock-repn-of-L2(S',P)}.
  \end{proof}
\end{lemma}
Alternatively, Lemma~\ref{thm:int(u)=0-over-bdG} holds because the expectation of every odd-power monomial vanishes by \eqref{eqn:Minlos-expectation-integral}; see also \eqref{eqn:expectation-of-even-monomials} and the surrounding discussion of Remark~\ref{rem:Wiener-improves-Minlos}.
Recall that we abuse notation and write $h_x = \la h_x, \cdot \ra_\Wiener = \tilde h_x$ for elements of $\Schw'$. 

\begin{defn}\label{def:mu_x}
  Denote the measure appearing in Corollary~\ref{thm:Boundary-integral-repn-for-harm} by    
  \linenopax
  \begin{equation}\label{eqn:def:boundary-kernel}
    d\gm_x := (\one + h_x) \, d\quotprob.  
  \end{equation}
  The function \one does not show up in \eqref{eqn:integral-boundary-repn-of-h} because it is orthogonal to \Harm:
\linenopax
\begin{align*}
  \int_{\Squoth} u (\one + h_x) \, d\quotprob
  = \int_{\Squoth} u \, d\quotprob + \la u, h_x\ra_\energy
  = \la u, h_x\ra_\energy,
  \qq\text{for } u \in \Harm,
\end{align*}
where we used Lemma~\ref{thm:int(u)=0-over-bdG}. Nonetheless, its presence is necessary, %otherwise 
%\linenopax
%  \begin{align*}%\label{eqn:}
%    \int_{\Schw'} h_x \,d\quotprob 
%    = \int_{\Schw'} \one h_x \,d\quotprob 
%    = \la h_x, \one\ra_\Wiener 
%  \end{align*}
\linenopax
\begin{align*}
  \int_{\Squoth} \one d\gm_x 
  &= \int_{\Squoth} \one (\one + h_x) \, d\quotprob 
  = \int_{\Squoth} \one \, d\quotprob  + \int_{\Squoth} \one h_x \, d\quotprob 
  %= 1 + \la h_x, \one\ra_\Wiener 
  = 1,
\end{align*}
again by Lemma~\ref{thm:int(u)=0-over-bdG}. 
\end{defn}

\begin{remark}\label{rem:kernel-nonnegative}
  \version{}{\marginpar{$\gm_x \geq 0$ or $h_x \geq 0$?}}
  We have shown that as a linear functional, $\gm_x[\one]=1$. It follows by standard functional analysis that $\gm_x \geq 0$ \quotprob-a.e. on $\Squoth $. Thus, $\gm_x$ is absolutely continuous with respect to \quotprob ($\gm_x \ll \quotprob$) with Radon-Nikodym derivative $\frac{d\gm_x}{d\quotprob} = \one + h_x$.
\end{remark}

\begin{comment}
  for reasons that can best be explained in terms of the Fock space representation of $L^2(\Squot,\quotprob)$ as the second quantization of \HE: the constant function \one corresponds to the vaccuum vector; see \cite[\S4]{Hida80} for more details. It is critical to observe that $\one = 0$ in \HE, but $\one \neq 0$ on $\Schw'$.
For every $x \in \verts$, 
\end{comment}



\begin{defn}\label{def:harmonic-equivalence-of-paths}
  Recall that a path in \Graph is an infinite sequence of successively adjacent vertices. We say that a path $\cpath = (x_0, x_1, x_2, \dots)$ is a \emph{path to infinity}, and write $\cpath \to \iy$, iff \cpath eventually leaves any finite set $F \ci \verts$, i.e.,
  \linenopax
  \begin{align}\label{eqn:def:path-to-infinity}
    \exists N \text{ such that } n \geq N \implies x_n \notin F.
  \end{align}
  
  If $\cpath_1 = (x_0, x_1, x_2, \dots)$ and $\cpath_2 = (y_0, y_1, y_2, \dots)$ are two paths to infinity, define an equivalence relation by    
  \linenopax
  \begin{equation}\label{eqn:def:harmonic-equivalence-of-paths}
    \cpath_1 \simeq \cpath_2
    \q\iff\q
    \lim_{n \to \iy} (h(x_n)-h(y_n)) = 0, \q\text{for every } h \in \MP.% / \Fin.
  \end{equation}
  In particular, all paths to infinity are equivalent when $\Harm = 0$.
\end{defn}
  \glossary{name={\cpath},description={path},sort=G}

If $\gb = [\cpath]$ is any such equivalence class, pick any path $\cpath = (x_0, x_1, x_2, \dots)$ representing this class, and consider the associated sequence of measures $\{\gm_{x_n}\}$. These probability measures lie in the unit ball in the weak-$\star$ topology, so Alaoglu's theorem gives a weak-$\star$ limit
  \linenopax
  \begin{equation}\label{eqn:def:prob-meas-corr-to-a-path}
    \gn_\gb := \lim_{n \to \iy} \gm_{x_n}.% \in Prob\left(\tfrac{\Schw'}{\Fin}\right).
  \end{equation}
For any $h \in \Harm$, this measure satisfies 
  \linenopax
  \begin{equation}\label{eqn:h(xn)-becomes-h(b)}
    h(x_{n}) = \int_{\Squoth} \tilde h \,d\gm_{x_n} 
    \limas{n} \int_{\bd \Graph} \tilde h \,d\gn_\gb.
  \end{equation}
Thus, we define $\bd \Graph$ to be the collection of all such \gb, and extend harmonic functions to $\bd \Graph$ via
  \linenopax
  \begin{equation}\label{eqn:def:h(b)}
    \tilde h(\gb) := \int_{\bd \Graph} \tilde h \,d\gn_\gb.
  \end{equation}

\begin{defn}\label{def:bounded-in-HE}
  For $u \in \HE$, denote $\|u\|_\iy := \sup_{x \in \verts} |u(x)-u(o)|$, and say $u$ is \emph{bounded} iff $\|u\|_\iy < \iy$.
\end{defn}

\begin{lemma}\label{thm:Pfin-preserves-boundedness}
  If $v \in \HE$ is bounded, then $\Pfin v$ is also bounded. Moreover, every $v \in \MP$ is bounded.
\end{lemma}


\begin{theorem}\label{thm:bdy-point-as-linear-fnl}
  Let $\gb \in \bd \Graph$ and let $\cpath = (x_0, x_1, x_2, \dots)$ is any representative of \gb.
  Then $\gb \in \bd \Graph$ defines a continuous linear functional on \Schw via
  \linenopax
  \begin{align}\label{eqn:bdy-pt-as-meas-limit-along-a-path}
    \gb(v) := \lim_{n \to \iy} \int_{\Schw'} \tilde v \, d\gm_{x_n}, 
    \qq v \in \Schw.
  \end{align}
  In fact, the action of \gb is equivalently given by 
  \linenopax
  \begin{align}\label{eqn:bdy-pt-as-eval-limit-along-a-path}
    \gb(v) = \lim_{n \to \iy} \Phar v({x_n})- \Phar v(o), 
    \qq v \in \Schw.
  \end{align}
\end{theorem}

\begin{remark}\label{rem:bdG-as-Diracs-at-infinity}
  In light of \eqref{eqn:bdy-pt-as-eval-limit-along-a-path}, one can think of $\gn_\gb$ in \eqref{eqn:def:prob-meas-corr-to-a-path} as a Dirac mass. Thus, $\gb \in \bd \Graph$ is a boundary point, and integrating a function $f$ against $\gn_\gb$ corresponds to evaluation of $f$ at that boundary point.
\end{remark}





